No Train Still Gain. Unleash Mathematical Reasoning of Large Language Models with Monte Carlo Tree Search Guided by Energy Function

Large language models (LLMs) demonstrate impressive language understanding and contextual learning abilities, making them suitable for natural language processing (NLP) tasks and complex mathematical reasoning. However, when applied to mathematical reasoning tasks, LLMs often struggle to generate correct reasoning steps and answers despite having high probabilities for the solutions. To overcome this limitation and enhance the mathematical reasoning capabilities of fine-tuned LLMs without additional fine-tuning steps, we propose a method that incorporates Monte Carlo Tree Search (MCTS) and a lightweight energy function to rank decision steps and enable immediate reaction and precise reasoning. Specifically, we re-formulate the fine-tuned LLMs into a Residual-based Energy Model (Residual-EBM) and employ noise contrastive estimation to estimate the energy function's parameters. We then utilize MCTS with the energy function as a path verifier to search the output space and evaluate the reasoning path. Through extensive experiments on two mathematical reasoning benchmarks, GSM8k and AQUA-RAT, we demonstrate the exceptional capabilities of our method, which significantly improves the pass@1 metric of the fine-tuned model without requiring additional fine-tuning or reinforcement learning with human feedback alignment.

==> Figures/Table_GSM8K_MATH_merge.tex <==


% In this study, to ensure equitable and cohesive evaluations, we report the socres of all models within the settings of greedy decoding and CoT~\cite{wei2022chain}.

\begin{table}
    \centering
    \caption{Results of pass@1 (\%) on GSM8k and MATH. In this study, to ensure equitable and cohesive evaluations, we report the socres of all models within the settings of greedy decoding and CoT~\cite{wei2022chain}. We report the improvement between WizardMath and baseline model with similar parameter size.}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} & \textbf{Params} & \textbf{GSM8k} & \textbf{MATH}  \\
        \midrule
        \multicolumn{4}{c}{Closed-source models}\\
        \midrule
        GPT-4 ~\cite{openai2023gpt4} & - & 92.0 & 42.5\\
        Claude 2\footref{fn:claude2} & - & 88.0 & -\\
        Claude 1.3\footref{fn:claude2} & - & 85.2 & -\\
        Flan-PaLM 2~\cite{palm2} & 540B & 84.7 & 33.2 \\
        Claude Instant\footref{fn:claude2} & - & 80.9 & -\\
        ChatGPT~\cite{zhao2023modelselection} & - & 80.8 & 34.1\\
        PaLM 2~\cite{palm2} & 540B & 80.7 & 34.3\\
        \midrule
        \multirow{3}{*}{Minerva~\cite{lewkowycz2022solving}} & 8B & 16.2 & 14.1\\
        & 62B & 52.4 & 27.6\\
        & 540B & 58.8 & 33.6
        \\\midrule
        GPT-3.5~\cite{openai2023gpt4} & - & 57.1 & -
        \\\midrule
        \multirow{3}{*}{PaLM~\cite{PaLM}} & 8B & 4.1 & 1.5\\
        & 62B & 33.0 & 4.4\\
        & 540B & 56.5 & 8.8
        \\\midrule
        RFT-13B ~\cite{yuan2023RFT} & 13B & 55.4 & -\\
        Chinchilla ~\cite{Chinchilla} & 70B & 43.7 & -\\
        ChatGLM 2~\cite{GLM-130B} & 12B & 40.9 & -\\
        Text-davinci-002 ~\cite{lewkowycz2022solving} & 175B & 40.7 & 19.1\\
        GPT-3~\cite{brown2020language} & 175B & 34.0 & 5.2\\
        GPT-2~\cite{hendrycks2021measuring} & 1.5B & - & 6.9\\
        \midrule
        \multicolumn{4}{c}{Open-source models}
        \\\midrule
        \multirow{2}{*}{GAL~\cite{taylor2022galactica}} & 30B & - & 12.7\\
        & 120B & - & 20.4
        \\\midrule
        \multirow{4}{*}{LLaMA 2~\cite{touvron2023llama2}} & 7B & 14.6 & 2.5\\
        & 13B & \underline{28.7} & \underline{3.9}\\
        & 34B & 42.2 & 6.24\\
        & 70B & \underline{56.8} & \underline{13.5}
        \\\midrule
        Qwen \footref{fn:qwen} & 7B & \underline{51.6} & -
        \\\midrule
        \multirow{4}{*}{LLaMA 1~\cite{touvron2023llama}} & 7B & 11.0 & 2.9\\
        & 13B & 17.8 & 3.9\\
        & 33B & 35.6 & 7.1\\
        & 65B & 50.9 & 10.6
        \\\midrule
        RFT-7B ~\cite{yuan2023RFT} & 7B & 50.3 & -\\
        GPT-J-6B ~\cite{gpt-j} & 6B & 34.9 & -\\
        ChatGLM 2~\cite{GLM-130B} & 6B & 32.4 & -\\
        InternLM-7B ~\cite{2023internlm} & 7B & 31.2 & -\\
        Vicuna v1.3 ~\cite{vicuna2023} & 13B & 27.6 & -\\
        Baichuan-chat \footref{fn:baichuan} & 13B & 23.9 & -
        \\\midrule
        \multirow{2}{*}{Falcon~\cite{penedo2023falcon}} & 7B & 6.8 & 2.3\\
        & 40B & 19.6 & 2.5
        \\\midrule
        GPT-Neo-2.7B ~\cite{Black2021GPTNeoLS} & 2.7B & 19.5 & -
        \\\midrule
        \multirow{2}{*}{MPT\footref{fn:mpt}} & 7B & 6.8 & \underline{3.0}\\
        & 30B & 15.2 & 3.1
        \\\midrule
        % WizardLM v1.2 ~\cite{xu2023wizardlm} & 13B & 55.4 & xxx\\
        % \midrule
        \emph{\textbf{WizardMath}} & 7B & \textbf{54.9} (\textcolor{red}{+3.3}) & \textbf{10.7} (\textcolor{red}{+7.7})\\
        \emph{\textbf{WizardMath}} & 13B & \textbf{63.9} (\textcolor{red}{+35.2}) & \textbf{14.0} (\textcolor{red}{+10.1})\\
        \emph{\textbf{WizardMath}} & 70B & \textbf{81.6} (\textcolor{red}{+24.8}) & \textbf{22.7} (\textcolor{red}{+9.2})\\
        \bottomrule
    \end{tabular}
    \label{tab:gsm8k_math_merge}
\end{table}

==> Figures/Tables/Table_GSM8K_MATH_merge.tex <==


% In this study, to ensure equitable and cohesive evaluations, we report the socres of all models within the settings of greedy decoding and CoT~\cite{wei2022chain}.

\begin{table}
    \centering
    \caption{Results of pass@1 (\%) on GSM8k and MATH. In this study, to ensure equitable and cohesive evaluations, we report the socres of all models within the settings of greedy decoding and CoT~\cite{wei2022chain}. We report the improvement between WizardMath and baseline model with similar parameter size.}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} & \textbf{Params} & \textbf{GSM8k} & \textbf{MATH}  \\
        \midrule
        \multicolumn{4}{c}{Closed-source models}\\
        \midrule
        GPT-4 ~\cite{openai2023gpt4} & - & 92.0 & 42.5\\
        Claude 2\footref{fn:claude2} & - & 88.0 & -\\
        Claude 1.3\footref{fn:claude2} & - & 85.2 & -\\
        Flan-PaLM 2~\cite{palm2} & 540B & 84.7 & 33.2 \\
        Claude Instant\footref{fn:claude2} & - & 80.9 & -\\
        ChatGPT~\cite{zhao2023modelselection} & - & 80.8 & 34.1\\
        PaLM 2~\cite{palm2} & 540B & 80.7 & 34.3\\
        \midrule
        \multirow{3}{*}{Minerva~\cite{lewkowycz2022solving}} & 8B & 16.2 & 14.1\\
        & 62B & 52.4 & 27.6\\
        & 540B & 58.8 & 33.6
        \\\midrule
        GPT-3.5~\cite{openai2023gpt4} & - & 57.1 & -
        \\\midrule
        \multirow{3}{*}{PaLM~\cite{PaLM}} & 8B & 4.1 & 1.5\\
        & 62B & 33.0 & 4.4\\
        & 540B & 56.5 & 8.8
        \\\midrule
        RFT-13B ~\cite{yuan2023RFT} & 13B & 55.4 & -\\
        Chinchilla ~\cite{Chinchilla} & 70B & 43.7 & -\\
        ChatGLM 2~\cite{GLM-130B} & 12B & 40.9 & -\\
        Text-davinci-002 ~\cite{lewkowycz2022solving} & 175B & 40.7 & 19.1\\
        GPT-3~\cite{brown2020language} & 175B & 34.0 & 5.2\\
        GPT-2~\cite{hendrycks2021measuring} & 1.5B & - & 6.9\\
        \midrule
        \multicolumn{4}{c}{Open-source models}
        \\\midrule
        \multirow{2}{*}{GAL~\cite{taylor2022galactica}} & 30B & - & 12.7\\
        & 120B & - & 20.4
        \\\midrule
        \multirow{4}{*}{LLaMA 2~\cite{touvron2023llama2}} & 7B & 14.6 & 2.5\\
        & 13B & \underline{28.7} & \underline{3.9}\\
        & 34B & 42.2 & 6.24\\
        & 70B & \underline{56.8} & \underline{13.5}
        \\\midrule
        Qwen \footref{fn:qwen} & 7B & \underline{51.6} & -
        \\\midrule
        \multirow{4}{*}{LLaMA 1~\cite{touvron2023llama}} & 7B & 11.0 & 2.9\\
        & 13B & 17.8 & 3.9\\
        & 33B & 35.6 & 7.1\\
        & 65B & 50.9 & 10.6
        \\\midrule
        RFT-7B ~\cite{yuan2023RFT} & 7B & 50.3 & -\\
        GPT-J-6B ~\cite{gpt-j} & 6B & 34.9 & -\\
        ChatGLM 2~\cite{GLM-130B} & 6B & 32.4 & -\\
        InternLM-7B ~\cite{2023internlm} & 7B & 31.2 & -\\
        Vicuna v1.3 ~\cite{vicuna2023} & 13B & 27.6 & -\\
        Baichuan-chat \footref{fn:baichuan} & 13B & 23.9 & -
        \\\midrule
        \multirow{2}{*}{Falcon~\cite{penedo2023falcon}} & 7B & 6.8 & 2.3\\
        & 40B & 19.6 & 2.5
        \\\midrule
        GPT-Neo-2.7B ~\cite{Black2021GPTNeoLS} & 2.7B & 19.5 & -
        \\\midrule
        \multirow{2}{*}{MPT\footref{fn:mpt}} & 7B & 6.8 & \underline{3.0}\\
        & 30B & 15.2 & 3.1
        \\\midrule
        % WizardLM v1.2 ~\cite{xu2023wizardlm} & 13B & 55.4 & xxx\\
        % \midrule
        \emph{\textbf{WizardMath}} & 7B & \textbf{54.9} (\textcolor{red}{+3.3}) & \textbf{10.7} (\textcolor{red}{+7.7})\\
        \emph{\textbf{WizardMath}} & 13B & \textbf{63.9} (\textcolor{red}{+35.2}) & \textbf{14.0} (\textcolor{red}{+10.1})\\
        \emph{\textbf{WizardMath}} & 70B & \textbf{81.6} (\textcolor{red}{+24.8}) & \textbf{22.7} (\textcolor{red}{+9.2})\\
        \bottomrule
    \end{tabular}
    \label{tab:gsm8k_math_merge}
\end{table}

==> Figures/Tables/math_topics.tex <==
\begin{table}
    \centering
    \caption{Results of pass@1 (\%) on MATH Subtopics with WizardMath 70B model.}
    \begin{tabular}{lccc}
        \toprule
        \textbf{MATH subtopics} & \textbf{WizardMath 70B}\\
        \midrule
        Intermediate Algebra & 7.1\\
        Precalculus & 12.6\\
        Geometry & 15.7\\
        Number Theory & 16.3\\
        Counting \& Probability & 17.3\\
        Prealgebra & 41.7\\
        Algebra & 33.3\\
        \midrule
        Overall & \textbf{22.7}\\
        \bottomrule
    \end{tabular}
    \label{tab:math_topics}
\end{table}
